Online Observability of Boolean Control Networks

Observabililty is an important topic of Boolean control networks (BCNs). In this paper, we propose a new type of observability named online observability to present the sufficient and necessary condition of determining the initial states of BCNs, when their initial states cannot be reset. And we design an algorithm to decide whether a BCN has the online observability. Moreover, we prove that a BCN is identifiable iff it satisfies controllability and the online observability, which reveals the essence of identification problem of BCNs.

==> sec/applications.tex <==
% !Mode\dots ``TeX:UTF-8''
% !TEX root = ../root.tex
\section{Optimization}
\label{sec:app}

%In the {\em Section \ref{sec:online}}, we present that t
%The online observability can help us determine the initial states of some \BCNs\ which can not be determined by the existing observability. In addition, 
We can also use the online observability to do some optimization in the process of determining the initial states of the \BCNs, including finding the shortest path and avoid entering critical states. 

\subsection{Finding shortest path}
An important aspect that we would consider is to find the shortest path to determine the initial state. In general, we can not find the shortest path definitely because the output is uncertain. Fortunately, we can use the input-labelled graph to make the best decision. For the path to determine the initial state of the \BCNs, we introduce two functions $\Pe(\mathsf{S},\mathsf{ i}^{i})$ and $\Pv(\mathsf{S},\mathsf{ i}^{i})$ to describe the expected value and variance for every vertex $\mathsf{S}$ of the input-labelled graph, respectively.% 

We introduce some necessary statements before defining the functions $\Pe(\mathsf{S},\mathsf{ i}^{i})$ and $\Pv(\mathsf{S},\mathsf{ i}^{i})$:
\begin{itemize}
  \item $\mathsf{S}$: the state set in a vertex of input-labelled graph;
  \item $\{\mathsf{ i}^{1},\mathsf{ i}^{2},\ldots, \mathsf{ i}^{p}\}$ : the inputs set of $\mathsf{S}$;
  \item $\{\mathsf{o}^1,\mathsf{o}^2,\ldots,\mathsf{o}^k\}$: the set of possible outputs of \BCN\ at next time point as we input $\mathsf{ i}^{i}$;
 \item $\{\mathsf{S}^{1},\mathsf{S}^{2},\ldots, \mathsf{S}^{k}\}$ : the set of possible state sets at next time point, where $\mathsf{S}^{j}=\Ded(\mathsf{S},\mathsf{i}^{i},\mathsf{o}^{j})$.
  
\end{itemize} 

Then $\Spe(\mathsf{S})$ and $\Pe(\mathsf{S},\mathsf{ i}^{i})$ are defined as follows.

\begin{definition}[$\Spe(\mathsf{S})$] \label{lspe}
\begin{equation}
\begin{split}
\Spe(\mathsf{S})= \min(\Pe(\mathsf{S}, \mathsf{ i}^{1}),\ldots,\Pe(\mathsf{S}, \mathsf{ i}^{p})).
\end{split}
\end{equation}
\end{definition}

\begin{definition}[$\Pe(\mathsf{S}, \mathsf{ i}^{i})$] \label{spe}

\[\Pe(\mathsf{S}, \mathsf{ i}^{i})=\left\{
\begin{array}{rcl}
0      &      & {|\mathsf{S}|=1}\\
1 +\frac{\sum_{j=1}^k \Spe(\mathsf{S}^{j})|\mathsf{S}^{j}|}{ |\mathsf{S}|}       &      & {|\mathsf{S}|>1}
\end{array} \right. \]

\end{definition}

The function $\Spe(\mathsf{S})$ is used to find the $\mathsf{ i}^{i}$ from $\{\mathsf{ i}^{1},\mathsf{ i}^{2},\ldots, \mathsf{ i}^{z}\}$ to calculat least $\Pe(\mathsf{S}, \mathsf{ i}^{i})$ for $\mathsf{S}$. In the definition of $\Pe(\mathsf{S}, \mathsf{ i}^{i})$, if $|\mathsf{S}|=1$ then we can determine $\mathsf{s}$. Thus we no longer need to choose the input to determine the state $\mathsf{s}$ of \BCNs. Therefore, for any input the path expected value $\Pe(\mathsf{S}, \mathsf{ i}^{i})$ would be $0$ and the shortest path expected value $\Spe(\mathsf{S})$ also would be $0$ too. While, if $|\mathsf{S}|>1$, then we still need to choose input and observe the output to determine the state of of \BCNs. Thus we recursively define the $\Pe(\mathsf{S}, \mathsf{ i}^{i})$ and $\Spe(\mathsf{S})$ for $\mathsf{S}$ and each input $\mathsf{ i}^{i}$ in the inputs set of $\mathsf{S}$. 

Such that, at every time point, with $\mathsf{S}(t)$ we derived, we can decide $\mathsf{i}(t)$ by $\Pe(\mathsf{S}(t),\mathsf{ i}(t))$ to try to find the shortest path. If we want to find the shortest path to determine the initial state of a \BCN, we can choose an input $\mathsf{ i}^{i}(t)$ with least $\Pe(\mathsf{S}(t), \mathsf{ i}^{i}(t))$. This input $\mathsf{i}^{i}(t)$ may help us find the shortes path to determine $\mathsf{s}(0)$. But the $\mathsf{o}(t)$ of \BCNs\ we observe is uncertain, hence selecting the $\mathsf{ i}^{i}(t)$ may leads to a very long path. For better performce, we define the $\Pv(\mathsf{S}, \mathsf{ i}^{i})$ to avoid risks.
\begin{definition}[$\Pv(\mathsf{S}, \mathsf{ i}^{i})$] 
\[\Pv(\mathsf{S}, \mathsf{ i}^{i})=\left\{
\begin{array}{rcl}
0      &      & {|\mathsf{S}|=1}\\
\frac{\sum_{j=1}^k (\Spe(\mathsf{S}^{j})-\Pe(\mathsf{S}, \mathsf{ i}^{i})+1)^2 |\mathsf{S}^{j}|}{ |\mathsf{S}|}      &      & {|\mathsf{S}|>1}
\end{array} \right. \]
\end{definition}

If the $\Pv(\mathsf{S}(t), \mathsf{i}^{i}(t))$ is not very large, the risk of choosing $\mathsf{ i}^{i}(t)$ would be not very great either.
%From the definition of the $\Pv(\mathsf{S}, \mathsf{ i}^{i})$, we have that 
\subsection{Avoiding entering critical states}
In biological systems wich depiected by the \BCNs, some of the states may corresponding to unfavorable or even dangerous situations \cite{Li2014Controllability}. So another important aspect that we consider in the process of determining the \BCN's initial state is to avoid entering critical states. Therefore, we also construct two functions $\Ce(\mathsf{S}, \mathsf{ i}^{i})$ and $\Cv(\mathsf{S}, \mathsf{ i}^{i})$ to describe expected value and variance of the times of entering critical states for every $\mathsf{S}$, respectively. 
%The definition of $\Lce(\mathsf{S})$ and $\Ce(\mathsf{S}, \mathsf{ i}^{i})$ are as follows.\\
\begin{definition}[$\Lce(\mathsf{S})$] \label{lce}
\begin{equation}
\begin{split}
\Lce(\mathsf{S})= \min(\Ce(\mathsf{S}, \mathsf{ i}^{1}),\ldots,\Ce(\mathsf{S}, \mathsf{ i}^{p})).
\end{split}
\end{equation}
\end{definition}
\begin{definition}[$\Ce(\mathsf{S}, \mathsf{ i}^{i})$] 
\[\Ce(\mathsf{S}, \mathsf{ i}^{i})=\left\{
\begin{array}{rcl}
|\mathsf{S} \cap \mathsf{S}_{cri} |      &      & {|\mathsf{S}|=1}\\
|\mathsf{S} \cap \mathsf{S}_{cri}| +\frac{\sum_{j=1}^k \Lce(\mathsf{S}^{j})|\mathsf{S}^{j}|}{ |\mathsf{S}|}     &      & {|\mathsf{S}|>1}
\end{array} \right. \]
where $\mathsf{S}_{cri}$ is the set of critical states.
\end{definition}

With the critical states set $\mathsf{S}_{cri}$, the definition of $\Ce(\mathsf{S}, \mathsf{ i}^{i})$ has some difference with $\Pe(\mathsf{S}, \mathsf{ i}^{i})$. We can analyze the possibility of entering the critical states by caculate $\Ce(\mathsf{S}, \mathsf{ i}^{i})$ for every vertex in the input-labelled graph. And we get the definitions of $\Cv(\mathsf{S}, \mathsf{ i}^{i})$ in the similar way.

\begin{definition}[$\Cv(\mathsf{S}, \mathsf{ i}^{i})$] 
\[\Cv(\mathsf{S}, \mathsf{ i}^{i})=\left\{
\begin{array}{rcl}
0     &      & {|\mathsf{S}|=1}\\
\sum_{j=1}^k\frac{ (\Lce(\mathsf{S}^{j})-\Ce(\mathsf{S}, \mathsf{ i}^{i})+|\mathsf{S} \cap \mathsf{S}_{cri}|)^2 |\mathsf{S}^{j}|}{ |\mathsf{S}|}    &      & {|\mathsf{S}|>1}
\end{array} \right. \]
\end{definition}

The use of $\Ce(\mathsf{S}, \mathsf{ i}^{i})$ and $\Cv(\mathsf{S}, \mathsf{ i}^{i})$ are similar to $\Pe(\mathsf{S}, \mathsf{ i}^{i})$ and $\Pv(\mathsf{S}, \mathsf{ i}^{i})$ respectively. At every time $t$, with $\mathsf{S}(t)$ we derived, we can decide $\mathsf{i}(t)$ by $ \Pe(\mathsf{S}(t), \mathsf{ i}(t))$, $\Pv(\mathsf{S}(t), \mathsf{ i}(t))$, $\Ce(\mathsf{S}(t), \mathsf{ i}(t))$ and $\Cv(\mathsf{S}(t), \mathsf{ i}(t))$.

However, in the four existing types of observability, we can not analyze the state of the \BCNs\ dynamically. Hence it would be hard to do some optimization in the process of determining the initial state of the \BCNs. Fortunately, this problem can be solved by the online observability better, thus it further illustrates the advantages of online observability.

==> sec/test.tex <==
\section{ssssss}
\label{sec;one}
ssssssss

ss

s

s
s

d
d
f

